Improving Iterative Text Revision by Learning Where to Edit from Other Revision Tasks

Iterative text revision improves text quality by fixing grammatical errors, rephrasing for better readability or contextual appropriateness, or reorganizing sentence structures throughout a document. Most recent research has focused on understanding and classifying different types of edits in the iterative revision process from human-written text instead of building accurate and robust systems for iterative text revision. In this work, we aim to build an end-to-end text revision system that can iteratively generate helpful edits by explicitly detecting editable spans (where-to-edit) with their corresponding edit intents and then instructing a revision model to revise the detected edit spans. Leveraging datasets from other related text editing NLP tasks, combined with the specification of editable spans, leads our system to more accurately model the process of iterative text refinement, as evidenced by empirical results and human evaluations. Our system significantly outperforms previous baselines on our text revision tasks and other standard text revision tasks, including grammatical error correction, text simplification, sentence fusion, and style transfer. Through extensive qualitative and quantitative analysis, we make vital connections between edit intentions and writing quality, and better computational modeling of iterative text revisions.

==> tab/humaneval_rq1.tex <==
\begin{table*}[]
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccccc|c}
\toprule
 &  \textbf{Revision Depth} &  \textbf{Overall Quality} &  \textbf{Fluency} &  \textbf{Coherence} &  \textbf{Meaning} &  \textbf{Readability} & \textbf{Total Documents} \\
\midrule
Human Edits                & 1 & -0.19 & -0.05 & \textbf{0.18}  & -0.31 & 0.13  & 22 \\
Human Edits                & 2 & -0.23 & \textbf{0.00}  & -0.23 & -0.69 & 0.09  & 22 \\
Human Edits                & 3 & -0.07 & 0.00  & -0.32 & -0.25 & 0.12  & 16 \\
\midrule
\iteraterbase \cite{du-etal-2022-understanding-iterative} 
                       & 1 & -0.14 & \textbf{0.31}  & -0.37 & -0.10 & -0.10 & 22 \\
\iteraterbase          & 2 & -0.17 & -0.06 & \textbf{-0.17} & 0.05  & -0.06 & 18 \\
\iteraterbase          & 3 & -0.38 & \textbf{0.18}  & -0.07 & 0.12  & 0.06  & 16 \\
\midrule
\textbf{\method} (Ours) & 1 & \textbf{0.18}  & -0.19 & -0.19 & \textbf{0.27}  & \textbf{0.63}  & 22 \\
\textbf{\method} & 2 & \textbf{-0.05} & -0.19 & -0.5  & \textbf{0.18}  & \textbf{0.09}  & 22 \\
\textbf{\method} & 3 & \textbf{0}     & -0.19 & \textbf{-0.05} & \textbf{0.13}  & \textbf{0.13}  & 22 \\

% Human Edits & 1 & 1.81 & 1.95 & 2.18 & 1.69 & 2.13 & 22  \\
% Human Edits & 2 & 1.77 & \textbf{2.00} & 1.77 & 1.31 & 2.09 & 22  \\
% Human Edits & 3 & 1.93 & 2.00 & 1.68 & 1.75 & 2.12 & 16  \\
% \midrule
% \iteraterbase \cite{du-etal-2022-understanding-iterative} & 1 & 1.86 & \textbf{2.31} & 1.63 & 1.90 & 1.90 & 22  \\
% \iteraterbase & 2 & 1.83 & 1.94 & \textbf{1.83} & 2.05 & 1.94 & 18  \\
% \iteraterbase  & 3 & 1.62 & \textbf{2.18} & \textbf{1.93} & 2.12 & 2.06 & 16  \\
% \midrule
% \textbf{\method} (Ours)  & 1 & \textbf{2.18} & 1.81 & 1.81 & \textbf{2.27} & \textbf{2.63} & 22  \\
% \textbf{\method}  & 2 & \textbf{1.95} & 1.81 & 1.5 & \textbf{2.18} & \textbf{2.09} & 22  \\
% \textbf{\method}  & 3 & \textbf{2} & 1.81 & \textbf{1.95} & \textbf{2.13} & \textbf{2.13} & 22 \\
\bottomrule
\end{tabular}
}
\caption{Manual pair-wise comparison for document revisions without Meaning-changed edits.}
\label{tab:human_rq1}
\vspace{-0.2cm}
\end{table*}


==> tab/intent_clf_results_sent_level.tex <==
\begin{table*}[t!]
\begin{center}
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccc|ccccc}
\midrule
& \multicolumn{5}{c}{\textbf{External Tasks}} & \multicolumn{5}{c}{\textbf{\iteraterbase-TEST}} \\
\midrule
& Clarity & Coherence & Fluency & Style & Overall & Clarity & Coherence & Fluency & Style & Overall \\
\midrule
SS:all & 96.00 & 100.00 & 97.00 & 97.00 & & 68.00 & 45.00 & 70.00 & 1.00 & 66.00 \\
SM:all & 95.00 & 100.00 & 99.00 & 97.00  & & 68.00 & 44.00 & 74.00 & 2.00 & 68.00 \\
MS:all & 93.00 & 100.00 & 98.00 & 96.00  & & 68.00 & 41.00 & 75.00 & 0.00 & 68.00 \\
MM:all & 96.00 & 100.00 & 97.00 & 97.00  & & 69.00 & 40.00 & 73.00 & 1.00 & 67.00 \\
SS:ext & 97.00 & 100.00 & 99.00 & 96.00  & & 50.00 & 7.00 & 34.00 & 2.00 & 37.00 \\
MS:200K & 89.00 & 16.00 & 67.00 & 0.00  & & 68.00 & 38.00 & 73.00 & 0.00 & 67.00 \\
Iterater & 60.00 & 16.00 & 73.00 & 0.00  & & 55.00 & 10.00 & 54.00 & 0.00 & 49.00 \\
\bottomrule
\end{tabular}
}
\caption{Performance of models on sentence-level intent classification.}
\label{tab:intent_clf_res_sent}
\end{center}
\end{table*}
